Sensitivity of Confinement Losses in Optical Fibers to Modeling Approach

A prime objective of modeling optical fibers is capturing mode confinement losses correctly. This paper demonstrates that specific modeling choices, especially regarding the outer fiber cladding regions and the placement of the computational boundary, have significant impacts on the calculated mode losses. Our results illustrate that one can obtain disparate mode confinement loss profiles for the same optical fiber design simply by moving the boundary to a new material region. We conclude with new recommendations for how to better model these losses.

==> figures/tikz/geom/zoomed.tex <==
    \begin{tikzpicture}
      [scale=0.125, show background rectangle,inner frame sep=0mm]

      \begin{scope}
        
        \clip (-20, 20) rectangle (20, 45); 
        
        % \fill [blue!30,even odd rule,opacity=0.6] (0,0)
        % circle[radius=68]
        % circle[radius=37.5];

        \fill [blue!30,even odd rule,opacity=0.6] (0,0)
        circle[radius=60]
        circle[radius=37.5];

        
        % % outer cladding layer
        % \draw[red, <->] (37.5,0) -- (68,0)
        % node [scale=0.75,black, midway, above] {{\tt{tclad}}};
        
        
        % The inner core region.
        \draw[red, dotted] (0,0) circle [radius=14.0];
        \draw[red, ->, dotted] (0,0) -- (14,0)
        node [scale=0.75,black, midway, above,fill=white] {{\tt{Rc}}};
        \fill[red] (0,0) circle (20pt);
        
        % The north capillary tube.
        \fill [blue!30,even odd rule,opacity=0.6] (0.0, 26.505) 
        circle [radius=12]
        circle [radius=10];
        
        % % Outer and inner radius of the capillary tubes.
        % \draw[red, ->] (0.0, 26.505) -- (0.0, 14.505)
        % node [scale=.75, black, midway, left] {{\tt{Rto}}}; 

        % \draw[->, red] (0.0, 26.505) -- (10.0, 26.505)
        % node [scale=0.75, black, midway, above] {{\tt{Rti}}};
        
        % Create a label for the distance that a given capillary
        % tube is embedded into the glass jacket.
        % \draw[-,red] (0.0, 37.505) -- (0.0, 38.505)
        % node [scale=0.75, black, above] {\tt{e*t}};
        
        % Create a label for the thickness of the capillary tubes.
        \draw[red, <->] (7.071067811865475, 33.57606781186547) --
        (8.48528137423857, 34.99028137423857) node [scale=0.75, black,
        above, right] {$\tc$}; % {$t$};
        
        % The northwest tube.
        \fill [blue!30,even odd rule,opacity=0.6] (-22.954003327306545, 13.2525) 
        circle [radius=12]
        circle [radius=10];
        
        % The southwest tube.
        \fill [blue!30,even odd rule,opacity=0.6] (-22.954003327306545,
        -13.2525) circle [radius=12] circle [radius=10];
        
        % A line to indicate the distance between any two capillary tubes.
        \draw[<->, red]
        (-22.954003327306545, 1.2525) -- (-22.954003327306545, -1.2525)
        node [scale=0.7, black, midway, right] {$\dc$};
        
        % The south tube.
        \fill [blue!30,even odd rule,opacity=0.6] (0.0, -26.505) 
        circle [radius=12]
        circle [radius=10];

        % The southeast tube.
        \fill [blue!30,even odd rule,opacity=0.6] (22.954003327306545, -13.2525) 
        circle [radius=12]
        circle [radius=10];

        % The northeast tube.
        \fill [blue!30,even odd rule,opacity=0.6] (22.954003327306545,
        13.2525) circle [radius=12] circle [radius=10];

        % Create a label for the distance that a given capillary
        % tube is embedded into the glass jacket.

        % \draw[-,red] (0.0, 37.505) -- (0.0, 38.505)
        % node [scale=0.75, black, above] {\tt{e*t}};

        \draw[->,red] (0.0, 35.505) -- (0.0, 37.505);
        \draw[->,red] (0.0, 40.505) -- (0.0, 38.505)
        node [scale=0.75, black, right] {$\ec$};

        
        % Outer and inner radius of the capillary tubes.
        \draw[->, red] (0.0, 26.505) -- (10.0, 26.505)
        node [scale=0.75, black, midway, above] {$\Rci$};

        \draw[red, ->] (0.0, 26.505) --++(-20:12)
        node [scale=.75, black, midway, sloped, below] {$\Rco$}; 
      \end{scope}
    \end{tikzpicture}

==> figures/tikz/mesh_compare/double/double.tex <==

\pgfplotstableread{figures/data/mesh_maxh/coarse_cladding1.dat}\coarseA
\pgfplotstableread{figures/data/mesh_maxh/coarse_cladding2.dat}\coarseB
\pgfplotstableread{figures/data/mesh_maxh/maxh_0.1_ref0.dat}\fineA
\pgfplotstableread{figures/data/mesh_maxh/maxh_0.1_ref1.dat}\fineB

\SetElement{\coarseA}{0}{1}{\ymin}
\SetElement{\coarseA}{0}{0}{\xmin}
\SetElement{\fineA}{0}{1}{\ymax}
\SetElement{\coarseA}{10}{0}{\coarseL}
\SetElement{\fineA}{5}{0}{\fineL}


\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=1 by 2,
            vertical sep=.9cm,
            xlabels at=edge bottom,
        },
        convergence_narrow,
        width=.89\textwidth,
        height=0.33\textwidth,
	    xlabel={Degrees of freedom},
	    ylabel={Loss (dB/m)},
	    ymode=log,
	    xmode=log,
	]
    \nextgroupplot[ymin=10^-6,
    						 ymax=10,
    						 xmin=\xmin, 
    						 xmax=3*10^6,
    						 title style={at={(0,1)},anchor=north west, yshift=-6},
    						 title={Naive Mesh},			 
    						 ]
%    						 
			\addplot +[mark=none, color=black!95, dashed, 
							  forget plot] coordinates {(\coarseL, 10^-8) (\coarseL, 100)};
%							  
			\addplot+[
			    color=orange!90!blue,
			    mark=*,
			    mark options={fill=orange!80!blue,},
			    mark size=.8pt,
			    line width=.85pt,
%			    skip coords between index={0}{1},
			    ]
			table[]{figures/data/mesh_maxh/coarse_cladding1.dat};
			\draw[very thick] (0,0) rectangle (.5,.5);

%%			
%			\SetElement{\coarseA}{0}{0}{\CAxa} \SetElement{\coarseA}{0}{1}{\CAya}
%			\node at (axis cs:\CAxa, \CAya) [pin={[font=\tiny, pin edge=
%			{solid, orange!80!blue}, orange!80!blue]0:\tiny $p=0$}]{};
%%
%			\SetElement{\coarseA}{14}{0}{\CAxb} \SetElement{\coarseA}{14}{1}{\CAyb}
%			\node at (axis cs:\CAxb, \CAyb) [pin={[font=\tiny, pin edge=
%			{solid, orange!80!blue}, orange!80!blue]-120:\tiny $p=14$}]{};
%%
%			\SetElement{\coarseA}{2}{0}{\CAxc} \SetElement{\coarseA}{2}{1}{\CAyc}
%			\node at (axis cs:\CAxc, \CAyc) [pin={[font=\tiny, pin edge=
%			{solid, orange!80!blue}, orange!80!blue]180:$p=2$}]{};
%%
			\addlegendentry{ref 0}
%			
%			
			\addplot+[
			    color=Blue!40,
			    mark=*,
			    mark options={fill=Blue!40},
			    mark size=.8pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/coarse_cladding2.dat};
%%			
%			\SetElement{\coarseB}{0}{0}{\CBxa} \SetElement{\coarseB}{0}{1}{\CBya}
%			\node at (axis cs:\CBxa, \CBya) [pin={[font=\tiny, pin edge=
%			{solid, Blue!40}, Blue!80]120:\tiny $p=0$}]{};
%%%
%			\SetElement{\coarseB}{9}{0}{\CBxb} \SetElement{\coarseB}{9}{1}{\CByb}
%			\node at (axis cs:\CBxb, \CByb) [pin={[font=\tiny, pin edge=
%			{solid, Blue!40}, Blue!80]-90:\tiny $p=9$}]{};
			\addlegendentry{ref 1}
%			
%
    \nextgroupplot[ymin=2*10^-2,
    						 ymax=5,
    						 xmin=\xmin, 
    						 xmax=3*10^6,
    						 title style={at={(0,1)},anchor=north west, yshift=-6},
    						 title={Informed Mesh},
   						 ]
			\addplot+[
			    color=orange!90!blue,
			    mark=*,
			    mark options={fill=orange!90!blue},
			    mark size=1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/maxh_0.1_ref0.dat};
			\addlegendentry{ref 0};
%			
%
			\addplot +[mark=none, color=black!95, dashed, 
							 forget plot] coordinates {(\fineL, .5\pgfkeysvalueof{/pgfplots/ymin}) 
							 (\fineL,2\pgfkeysvalueof{/pgfplots/ymax})};
%
%
%			\SetElement{\fineA}{0}{0}{\FAxa} \SetElement{\fineA}{0}{1}{\FAya}
%			\node at (axis cs:\FAxa,\FAya) [pin={[font=\tiny, pin edge=
%			{solid, orange!90!blue}, orange!90!blue]-135:\tiny $p=0$}]{};
%%			
%			\SetElement{\fineA}{12}{0}{\FAxb} \SetElement{\fineA}{12}{1}{\FAyb}
%			\node at (axis cs:\FAxb,\FAyb) [pin={[font=\tiny, pin edge=
%			{solid, orange!90!blue},orange!90!blue]120:\tiny $p=8$}]{};
%%%
%			\SetElement{\fineA}{2}{0}{\FAxc} \SetElement{\fineA}{2}{1}{\FAyc}
%			\node at (axis cs:\FAxc,\FAyc) [pin={[font=\tiny, pin edge={solid, blue}, blue]-87.5:$p=2$}]{};
%%
%			\SetElement{\coarseB}{2}{0}{\CBxc} \SetElement{\coarseB}{2}{1}{\CByc}
%			\node at (axis cs:\CBxc, \CByc) [pin={[font=\tiny, pin edge=
%         {solid, orange!80!blue}, orange!80!blue]100:$p=2$}]{};
%%			
			\addplot+[
			    color=Blue!40,
			    mark=*,
			    mark options={fill=Blue!40},
			    mark size=1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/maxh_0.1_ref1.dat};
%			\SetElement{\fineB}{0}{0}{\FBxa} \SetElement{\fineB}{0}{1}{\FBya}
%			\node at (axis cs:\FBxa,\FBya) [pin={[font=\tiny, pin edge=
%			{solid, Blue!40}, Blue!80]-120:$p=0$}]{};
%%%			
%			\SetElement{\fineB}{7}{0}{\FBxb} \SetElement{\fineB}{7}{1}{\FByb}
%			\node at (axis cs:\FBxb,\FByb) [pin={[font=\tiny, pin edge=
%			{solid, Blue!40}, Blue!80]-100:\tiny $p=4$}]{};
%%			
%			\SetElement{\fineB}{2}{0}{\FBxc} \SetElement{\fineB}{2}{1}{\FByc}
%			\node at (axis cs:\FBxc,\FByc) [pin={[font=\tiny, pin edge={solid, blue}, blue]-80:$p=2$}]{};
%			
			\addlegendentry{ref 1}
    \end{groupplot}
\end{tikzpicture}


==> figures/tikz/mesh_compare/double/pre.tex <==
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Ect}{\tilde{\mathcal{E}}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Sct}{\tilde{\mathcal{S}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Vct}{\tilde{\mathcal{V}}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\ii}{\hat{\imath}}
\newcommand{\SNa}{S_N^a}
\newcommand{\ut}{\tilde{u}}
\newcommand{\uh}{\hat{u}}
\newcommand{\vt}{\tilde{v}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\xh}{\hat{x}}
\newcommand{\yt}{\tilde{y}}
\newcommand{\Rt}{\tilde{R}}
\newcommand{\St}{\tilde{S}}
\newcommand{\Sm}[1]{S^{({#1})}}
\newcommand{\Pt}{\tilde{P}}
\newcommand{\Et}{\tilde{E}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Vt}{\tilde{V}}
\newcommand{\Wt}{\tilde{W}}
\newcommand{\vL}{\varLambda}
\newcommand{\veps}{\varepsilon}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\diam}{\mathop{\mathrm{diam}}}
\renewcommand{\Gamma}{\varGamma}
\renewcommand{\Lambda}{\varLambda}
\renewcommand{\vL}{\varLambda}
\newcommand{\vG}{\varGamma}
\newcommand{\ran}{\mathop{\mathrm{ran}}}
\newcommand{\Rh}{{\hat{R}}}
\newcommand{\rh}{{\hat{r}}}
\newcommand{\rt}{{\tilde{r}}}
\newcommand{\ec}{e_{\mathrm{cap}}}
\newcommand{\tc}{t_{\mathrm{cap}}}
\newcommand{\dc}{d_{\mathrm{cap}}}
\newcommand{\Rci}{R_{i, \mathrm{cap}}}
\newcommand{\Rco}{R_{o, \mathrm{cap}}}
\newcommand{\Rcore}{R_{\mathrm{core}}}
\newcommand{\tclad}{t_{\mathrm{clad}}}
\newcommand{\Rout}{\Rh_{\mathrm{fin}}}
\newcommand{\Rfin}{\Rh_{\mathrm{fin}}}
\newcommand{\og}{\omega}
\newcommand{\om}{\varOmega}
\newcommand{\oh}{\varOmega_h}
\newcommand{\nair}{{n_{\mathrm{air}}}}
\newcommand{\nsi}{{n_{\mathrm{Si}}}}
\newcommand{\omsi}{{\varOmega_{\mathrm{Si}}}}
\newcommand{\ompml}{{\varOmega_{\mathrm{pml}}}}
\newcommand{\omint}{{\varOmega_{\mathrm{int}}}}
\newcommand{\Ho}{\mathring{H}}
\newcommand{\Nedelec}{N{\'{e}}d{\'{e}}lec } 

\renewcommand{\AA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\vpt}{\tilde{\varphi}}

\newcommand{\Eth}{E^{h}_\tau}
\newcommand{\vph}{\varphi^{h}}
\newcommand{\vphi}{\varphi}
\newcommand{\Vhp}{\mathcal{V}^{h}}
\newcommand{\Nhp}{\mathcal{N}^{h}}
\newcommand{\nN}{n_\mathcal{N}}
\newcommand{\nV}{n_\mathcal{V}}

\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\dive}{div}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\grad}{grad}
\renewcommand{\d}{\partial}

\def\d{\partial}
\renewcommand{\Im}{\mathop{\mathrm{imag}}}
\renewcommand{\Re}{\mathop{\mathrm{real}}}
\newcommand{\jmp}[1]{\ldbrack{{#1}}\rdbrack}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "polyfeast"
%%% End:


==> figures/tikz/mesh_compare/single/single.tex <==
\pgfplotstableread{figures/data/mesh_maxh/mesh_maxh0.dat}\coarseA
\pgfplotstableread{figures/data/mesh_maxh/mesh_maxh2.dat}\fineA
\pgfplotstableread{figures/data/mesh_maxh/mesh_maxh1.dat}\fineB
\pgfplotstableread{figures/data/mesh_maxh/mesh_maxh3.dat}\fineC

\SetElement{\coarseA}{0}{1}{\ymin}
\SetElement{\coarseA}{0}{0}{\xmin}
\SetElement{\fineA}{0}{1}{\ymax}

	\begin{tikzpicture}
		\begin{axis}[convergence,
			width=.85\textwidth,
			height=.45\textwidth,
		    xlabel={Degrees of freedom},
		    ylabel={Confinement Loss [dB/m]},
		    ymode=log,
		    xmode=log]
%
			\addplot+[
			    color=red!80!blue,
			    mark=*,
			    mark size=1.1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/mesh_maxh0.dat};
			\SetElement{\coarseA}{11}{0}{\CAxa} \SetElement{\coarseA}{11}{1}{\CAya}
			\node at (axis cs:\CAxa, \CAya) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, red!80!blue]-70:$p=11$}]{};
%
%			\SetElement{\coarseA}{1}{0}{\CAxb} \SetElement{\coarseA}{1}{1}{\CAyb}
%			\node at (axis cs:\CAxb, \CAyb) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]145:$p=1$}]{};
%%			
%			\SetElement{\coarseA}{2}{0}{\CAxc} \SetElement{\coarseA}{2}{1}{\CAyc}
%			\node at (axis cs:\CAxc, \CAyc) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]180:$p=2$}]{};
%%
%			\SetElement{\coarseA}{3}{0}{\CAxd} \SetElement{\coarseA}{3}{1}{\CAyd}
%			\node at (axis cs:\CAxd, \CAyd) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]-92:$p=3$}]{};
%					
			\addlegendentry{0.3 $\lambda/h$}
%
			\addplot+[
			    color=orange,
			    mark=*,
			    mark size=1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/mesh_maxh1.dat};
			\SetElement{\fineB}{5}{0}{\FBxa} \SetElement{\fineB}{5}{1}{\FBya}
			\node at (axis cs:\FBxa,\FBya) [pin={[font=\tiny, pin edge={solid, orange}, orange]-110:$p=5$}]{};
%			
%			\SetElement{\fineB}{1}{0}{\FBxb} \SetElement{\fineB}{1}{1}{\FByb}
%			\node at (axis cs:\FBxb,\FByb) [pin={[font=\tiny, pin edge={solid, blue}, blue]87.7:$p=1$}]{};
%%			
%			\SetElement{\fineB}{2}{0}{\FBxc} \SetElement{\fineB}{2}{1}{\FByc}
%			\node at (axis cs:\FBxc,\FByc) [pin={[font=\tiny, pin edge={solid, blue}, blue]-92:$p=2$}]{};
%%			
%			\SetElement{\fineB}{3}{0}{\FBxd} \SetElement{\fineB}{3}{1}{\FByd}
%			\node at (axis cs:\FBxd,\FByd) [pin={[font=\tiny, pin edge={solid, blue}, blue]-88:$p=3$}]{};
%			
			\addlegendentry{0.9 $\lambda/h$}
%			
			\addplot+[
			    color=blue,
			    mark=*,
			    mark size=1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/mesh_maxh2.dat};
			\SetElement{\fineA}{3}{0}{\FAxa} \SetElement{\fineA}{3}{1}{\FAya}
			\node at (axis cs:\FAxa,\FAya) [pin={[font=\tiny, pin edge={solid, blue}, blue]-90:$p=3$}]{};
%			
%			\SetElement{\fineA}{1}{0}{\FAxb} \SetElement{\fineA}{1}{1}{\FAyb}
%			\node at (axis cs:\FAxb,\FAyb) [pin={[font=\tiny, pin edge={solid, blue}, blue]87.7:$p=1$}]{};
%%			
%			\SetElement{\fineA}{2}{0}{\FAxc} \SetElement{\fineA}{2}{1}{\FAyc}
%			\node at (axis cs:\FAxc,\FAyc) [pin={[font=\tiny, pin edge={solid, blue}, blue]-92:$p=2$}]{};
%%			
%			\SetElement{\fineA}{3}{0}{\FAxd} \SetElement{\fineA}{3}{1}{\FAyd}
%			\node at (axis cs:\FAxd,\FAyd) [pin={[font=\tiny, pin edge={solid, blue}, blue]-88:$p=3$}]{};
%%			
			\addlegendentry{1.5 $\lambda/h$}
			
			\addplot+[
			    color=green!80!blue,
			    mark=*,
			    mark size=1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/mesh_maxh/mesh_maxh3.dat};
			\SetElement{\fineC}{2}{0}{\FCxa} \SetElement{\fineC}{2}{1}{\FCya}
			\node at (axis cs:\FCxa,\FCya) [pin={[font=\tiny, pin edge={solid, green!80!blue}, green!80!blue]80:$p=2$}]{};
%			
%			\SetElement{\fineB}{1}{0}{\FBxb} \SetElement{\fineB}{1}{1}{\FByb}
%			\node at (axis cs:\FBxb,\FByb) [pin={[font=\tiny, pin edge={solid, blue}, blue]87.7:$p=1$}]{};
%%			
%			\SetElement{\fineB}{2}{0}{\FBxc} \SetElement{\fineB}{2}{1}{\FByc}
%			\node at (axis cs:\FBxc,\FByc) [pin={[font=\tiny, pin edge={solid, blue}, blue]-92:$p=2$}]{};
%%			
%			\SetElement{\fineB}{3}{0}{\FBxd} \SetElement{\fineB}{3}{1}{\FByd}
%			\node at (axis cs:\FBxd,\FByd) [pin={[font=\tiny, pin edge={solid, blue}, blue]-88:$p=3$}]{};
%			
			\addlegendentry{3 $\lambda/h$}    
%			
		\end{axis}
	\end{tikzpicture}

==> figures/tikz/mesh_compare/single2/single2.tex <==
	\begin{tikzpicture}
		\begin{axis}[convergence,
			width=.9\textwidth,
			height=.575\textwidth,
		    xlabel={Small random change},
		    ylabel={Confinement Loss [dB/m]},
		    ymode=log,
		    xmode=log]
%		    
			\addplot+[
			    color=blue,
			    mark=*,
			    mark size=1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/fine_cladding1.dat};
			\SetElement{\fineA}{0}{0}{\FAxa} \SetElement{\fineA}{0}{1}{\FAya}
			\node at (axis cs:\FAxa,\FAya) [pin={[font=\tiny, pin edge={solid, blue}, blue]180:$p=0$}]{};
%			
			\SetElement{\fineA}{1}{0}{\FAxb} \SetElement{\fineA}{1}{1}{\FAyb}
			\node at (axis cs:\FAxb,\FAyb) [pin={[font=\tiny, pin edge={solid, blue}, blue]87.7:$p=1$}]{};
%			
			\SetElement{\fineA}{2}{0}{\FAxc} \SetElement{\fineA}{2}{1}{\FAyc}
			\node at (axis cs:\FAxc,\FAyc) [pin={[font=\tiny, pin edge={solid, blue}, blue]-92:$p=2$}]{};
%			
			\SetElement{\fineA}{3}{0}{\FAxd} \SetElement{\fineA}{3}{1}{\FAyd}
			\node at (axis cs:\FAxd,\FAyd) [pin={[font=\tiny, pin edge={solid, blue}, blue]-88:$p=3$}]{};
%			
			\addlegendentry{fine}
%			
			\addplot+[
			    color=orange!90!blue,
			    mark=*,
			    mark size=1.1pt,
			    line width=.85pt,
			    ]
			table[]{figures/data/coarse_cladding1.dat};
			\SetElement{\coarseA}{0}{0}{\CAxa} \SetElement{\coarseA}{0}{1}{\CAya}
			\node at (axis cs:\CAxa, \CAya) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]0:$p=0$}]{};
%			
			\SetElement{\coarseA}{1}{0}{\CAxb} \SetElement{\coarseA}{1}{1}{\CAyb}
			\node at (axis cs:\CAxb, \CAyb) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]145:$p=1$}]{};
%			
			\SetElement{\coarseA}{2}{0}{\CAxc} \SetElement{\coarseA}{2}{1}{\CAyc}
			\node at (axis cs:\CAxc, \CAyc) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]180:$p=2$}]{};
%
			\SetElement{\coarseA}{3}{0}{\CAxd} \SetElement{\coarseA}{3}{1}{\CAyd}
			\node at (axis cs:\CAxd, \CAyd) [pin={[font=\tiny, pin edge={solid, orange!80!blue}, orange!80!blue]-92:$p=3$}]{};
%					
			\addlegendentry{coarse}
%
		\end{axis}
	\end{tikzpicture}


==> figures/tikz/wlstudies/arf/8tube/C0C1_w_subint.tex <==

\pgfplotstableread{figures/data/arf/6tube/C1_subinterval.dat}\Czerosub

\SetElement{\Czerosub}{0}{0}{\xmin}
\pgfplotstablegetrowsof{\Czerosub}
\pgfplotstablegetelem{\the\numexpr\pgfplotsretval-1}{0}\of{\Czerosub} \let\xmax\pgfplotsretval

\newcommand{\findYlims}[1]{%
\pgfplotstablegetrowsof{#1}
	\pgfmathtruncatemacro{\LastRowNo}{\pgfplotsretval-1}
\pgfplotstablesort[sort key={1}]{\sorted}{#1}%
    \pgfplotstablegetelem{\LastRowNo}{1}\of{\sorted}%
\xdef\Ymax{\pgfplotsretval}%
    \pgfplotstablegetelem{0}{1}\of{\sorted}%
\xdef\Ymin{\pgfplotsretval}}

\findYlims{\Czerosub}

\newcommand{\yscaling}{.05}

\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=1 by 2,
            vertical sep=.6cm,
            xlabels at=edge bottom,
        },
        wavelength,
	    ymode=log,
		legend style={legend pos=south east, font=\tiny},
	]
    \nextgroupplot[width=\textwidth,
    						 height=.45\textwidth,
        					 enlarge x limits=0.04,
	    					 enlarge y limits=0.04,
			x tick label style={font=\tiny, /pgf/number format/precision=1},
    						 ]
%							  
\draw[very thin, black!50] (axis cs:\xmin, \Ymin-\yscaling*\Ymin) rectangle (axis cs:\xmax, \Ymax + \yscaling*\Ymax);
		\coordinate (UL) at (axis cs:\xmin,\Ymax + \yscaling*\Ymax);
		\coordinate (UR) at (axis cs:\xmax,\Ymax + \yscaling*\Ymax);
			\addplot+[
			    color=blue!75,
			    enlargelimits=0.0,
			    mark=*,
			    mark options={fill=orange!80!blue,},
			    mark size=0pt,
			    line width=.1pt,
			    ]
			table[]{figures/data/arf/6tube/C1L.dat};
			\addlegendentry{$C_1$}
%			
%			
			\addplot+[
			    color=Green,
	    		enlarge y limits=.05,
			    mark=*,
			    mark options={fill=Blue!40},
			    mark size=0pt,
			    line width=.1pt,
			    forget plot,
			    ]
			table[]{figures/data/arf/6tube/C1_subinterval.dat};
%			\addlegendentry{p=6}
%			
			\addplot+[
			    color=blue!75,
			    enlargelimits=0.0,
			    mark=*,
			    mark options={fill=orange!80!blue,},
			    mark size=0pt,
			    line width=.1pt,
			    forget plot,
			    ]
			table[]{figures/data/arf/6tube/C1R.dat};
%			\addlegendentry{p=5}
%
			\addplot+[
			    color=BrickRed,
			    enlargelimits=0.0,
			    mark=*,
			    mark options={fill=orange!80!blue,},
			    mark size=0pt,
			    line width=.8pt,
			    ]
			table[]{figures/data/arf/6tube/C0.dat};
			\addlegendentry{$C_0$}
%
    \nextgroupplot[width=\textwidth,
    						 height=.3\textwidth,
	    					 enlarge y limits=\yscaling,
	    					 enlarge x limits=0,
						     xmin=\xmin,
						     xmax=\xmax,
		x tick label style={font=\tiny, /pgf/number format/zerofill=false,  /pgf/number format/precision=3},
			       			 ]
			\addplot+[
			    color=Green,
			    mark=*,
			    mark options={fill=orange!90!blue},
			    mark size=0pt,
			    line width=.5pt,
			    ]
			table[]{figures/data/arf/6tube/C1_subinterval.dat};
%			
			\addplot+[
			    color=BrickRed,
			    mark=*,
			    mark options={fill=orange!90!blue},
			    mark size=0pt,
			    line width=.8pt,
			    ]
			table[]{figures/data/arf/6tube/C0_subinterval.dat};
%			
		\end{groupplot}
%			
\draw[very thin, black!50] 
	(UL) -- (group c1r2.north west) node {};
\draw[very thin, black!50] 
	(UR) -- (group c1r2.north east) node {};
\end{tikzpicture}

==> figures/tikz/wlstudies/arf/8tube/residual_plot.tex <==
	\begin{tikzpicture}
		\begin{axis}[wavelength,
		    ymode=log,
		    enlargelimits=.05,
		    width=.95\textwidth,
		    height=.4\textwidth,
			legend style={legend pos=outer north east, font=\tiny},
		    ]
%
			\addplot+[
			    color=blue,
			    mark=*,
			    mark size=0pt,
			    line width=.001pt,
			    ]
			table[]{figures/data/arf/8tube/N3config_ref0.dat};
			\addlegendentry{$C_1$}
%			
			\addplot+[
			    color=BrickRed,
			    mark=*,
			    mark size=0pt,
			    line width=.75pt,
			    ]
			table[]{figures/data/arf/8tube/N2config.dat};
			\addlegendentry{$C_0$}
		\end{axis}
%		
	\end{tikzpicture}


==> figures/tikz/wlstudies/bragg/ref6tube.tex <==
	\begin{tikzpicture}
		\begin{axis}[wavelength,
		    ymode=log,
		    enlargelimits=.05,
		    ]
%
			\addplot+[
			    color=green!10!blue,
			    mark=*,
			    mark size=0pt,
			    line width=.75pt,
			    ]
			table[]{figures/data/bragg/6tube/analytic.dat};
		\end{axis}
	\end{tikzpicture}


==> figures/tikz/wlstudies/bragg/ref8tube.tex <==
	\begin{tikzpicture}
		\begin{axis}[wavelength,
		    ymode=log,
		   	ylabel={},
		    enlargelimits=.05,
		    ]
%
			\addplot+[
			    color=orange,
			    mark=*,
			    mark size=0pt,
			    line width=.75pt,
			    ]
			table[]{figures/data/bragg/8tube/analytic.dat};

		\end{axis}
	\end{tikzpicture}
